Quantifying Retriever-Generator Alignment in RAG with Local Explanations

Retrieval-Augmented Generation (RAG) systems combine dense retrievers and language models to ground outputs in external documents. However, the interaction between these components remains opaque, creating challenges for deployment in high-stakes domains. We present RAG-E, an end-to-end explainability framework that quantifies retriever-generator alignment through mathematically grounded attribution methods. Our approach adapts Integrated Gradients for retriever analysis, proposes a Monte Carlo-stabilized Shapley Value approximation for generator attribution, and introduces the Weighted Alignment between Retriever and Generator (WARG) metric to measure how closely the generator's document usage aligns with retriever rankings. Experiments on PopQA, QAMPARI, and TREC CAST datasets reveal substantial misalignment: depending on the model and setting, generators often ignore top-ranked documents and rely on documents ranked as less relevant. We show that WARG captures retriever-generator alignment better than Pearson and Spearman correlations and can serve as an indicator of RAG performance. RAG-E and WARG provide a practical framework for auditing this interaction, enabling more reliable and transparent RAG systems.

==> macros.tex <==
\usepackage{enumitem}
\usepackage[most]{tcolorbox}
\usepackage{array}
\usepackage{tabularx}

\makeatletter
\newcommand{\resizetable}[3][5pt]{%
\setlength{\tabcolsep}{0pt}%
\begin{tabular}{c}%
\resizebox{#2}{!}{\setlength{\tabcolsep}{#1}#3}\\%
\end{tabular}%
}
\newcommand{\shap}[1]{\textsc{#1}SHAP}
\newcommand{\xrag}{RAG-E}
\newcommand{\ret}{\textsc{Ret}}
\newcommand{\gen}{\textsc{Gen}}

\newcommand{\tok}[2]{%
  \tcbox[colback=#1,colframe=#1,boxsep=0pt,left=-1pt,right=-1pt,top=0pt,bottom=0pt,arc=1.5pt]{\strut{}#2}%
  \hspace{-3pt}%
}

\DeclareRobustCommand{\gradlegend}{%
  \begin{tikzpicture}[baseline=(n.base)]
    \node[inner sep=2.5pt, rounded corners=2pt, font=\small] (n) {\phantom{Only \ret{}\quad$\rightarrow$\quad Only \gen{}}};
    \shade[rounded corners=2pt, left color=cyan!85, right color=magenta!85] (n.south west) rectangle (n.north east);
    \node[inner sep=2.5pt, rounded corners=2pt, font=\small] at (n.center) {Only \ret{}\quad$\rightarrow$\quad Only \gen{}};
  \end{tikzpicture}%
}

\newcommand{\docchip}[3]{%
  \tcbox[colback=#1,colframe=#1,boxsep=1.5pt,left=3pt,right=3pt,top=2pt,bottom=2pt,arc=2pt]{%
    \begin{minipage}{30pt}
      \centering\small \textit{#2}\\[-1pt]
      \small (#3)
    \end{minipage}
  }%
}

\definecolor{Tab0}{HTML}{1f77b4}
\definecolor{Tab1}{HTML}{ff7f0e}
\definecolor{Tab2}{HTML}{2ca02c}
\definecolor{Tab3}{HTML}{d62728}
\definecolor{Tab4}{HTML}{9467bd}
\definecolor{Tab5}{HTML}{8c564b}
\definecolor{Tab6}{HTML}{e377c2}
\definecolor{Tab7}{HTML}{7f7f7f}
\definecolor{Tab8}{HTML}{bcbd22}
\definecolor{Tab9}{HTML}{17becf}

\newcounter{@questions}
\newcommand{\questionref}[1]{\hyperref[#1]{\textsc{rq}}}
\newcommand{\question}[2]{%
    \setlength{\tabcolsep}{2pt}
    \smallskip%
    \noindent%
    \begin{tabularx}{.99\linewidth}{lX}
        \refstepcounter{@questions}%
        \textbf{\textsc{rq}\label{#1}:}&%
        \textit{#2}\\
    \end{tabularx}%
    \smallskip
}

\newcommand{\anonymous}[2][]{
    \ifdefined\acl@anonymizetrue{#2}
    \else{#1}
    \fi
}

\setlist[itemize]{leftmargin=1.25em}
\setlist[enumerate]{leftmargin=1.25em}

\newtheorem{definition}{Definition}

\makeatother
\raggedbottom
